Thermoelectric transport properties of electron doped pyrite FeS2

Pyrite FeS$_2$ has been investigated for a wide range of applications, including thermoelectrics due to previous observation of large thermopower at room-temperature. However, the values of thermopower reported in the literature is extremely sensitive to the nature of sample -- whether they are natural or lab grown, bulk crystals or thin films -- and an ambiguity in the magnitude and sign of thermopower of pure FeS$_2$ exists. Variation in the magnitude of room-temperature thermopower has also been observed in Co-doped samples. Therefore, it is of interest to clarify the intrinsic thermopower of this system that could be measured in more pure samples. In this paper, we investigate the thermoelectric properties of Co-doped FeS$_2$ using first principles calculations. We apply three different doping schemes to understand the effect of electron doping in FeS$_2$, namely explicit Co-substitution, jellium doping and electron addition within rigid band approximation (RBA) picture. The calculated thermopower is less than $-50$ $\mu$V/K for all values of Co doping that we studied, suggesting that this system may not be useful in thermoelectric applications. Interestingly, we find that RBA substantially overestimates the magnitude of calculated thermopower compared to the explicit Co-substitution and jellium doping schemes. The overestimation occurs because the changes in the electronic structure due to doping-induced structural modification and charge screening is not taken into account by the rigid shift of the Fermi level within RBA. RBA is frequently used in first principles investigations of the thermopower of doped semiconductors, and Co-substituted FeS$_2$ illustrates a case where it fails.

==> preamble.tex <==
\usepackage{amsthm}
\usepackage{mathtools}
\usepackage{physics}
\usepackage{xcolor}
\usepackage{graphicx}
\usepackage[left=23mm,right=13mm,top=35mm,columnsep=15pt]{geometry} 
\usepackage{adjustbox}
\usepackage{placeins}
\usepackage[T1]{fontenc}
\usepackage{lipsum}
\usepackage{csquotes}
\usepackage{caption}
\usepackage{indentfirst}

